Decomposing causality into its synergistic, unique, and redundant components

Causality lies at the heart of scientific inquiry, serving as the fundamental basis for understanding interactions among variables in physical systems. Despite its central role, current methods for causal inference face significant challenges due to nonlinear dependencies, stochastic interactions, self-causation, collider effects, and influences from exogenous factors, among others. While existing methods can effectively address some of these challenges, no single approach has successfully integrated all these aspects. Here, we address these challenges with SURD: Synergistic-Unique-Redundant Decomposition of causality. SURD quantifies causality as the increments of redundant, unique, and synergistic information gained about future events from past observations. The formulation is non-intrusive and applicable to both computational and experimental investigations, even when samples are scarce. We benchmark SURD in scenarios that pose significant challenges for causal inference and demonstrate that it offers a more reliable quantification of causality compared to previous methods.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> preamble.tex <==
\usepackage[affil-it]{authblk}
\usepackage{titlesec} % For customizing section titles
\usepackage{setspace} % For adjusting line spacing
\usepackage[twoside,
            letterpaper,includeheadfoot,%
            layoutsize={8.125in,10.875in},%
            layouthoffset=0.1875in,%
            layoutvoffset=0.0625in,%
            left=38.5pt,%
            right=43pt,%
            top=43pt, % 10pt provided by headsep
            bottom=32pt,%
            headheight=0pt, % No Header
            headsep=10pt,%
            footskip=25pt,
            marginparwidth=38pt]{geometry}

\usepackage{lmodern} % Ensure Latin Modern Sans Serif is used
% \renewcommand{\familydefault}{\sfdefault}

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{xcolor}
% \usepackage{bm}
% \usepackage{amsbsy}
\usepackage{fixmath}
\usepackage{subcaption}
\usepackage{adjustbox}
\usepackage{pifont}
\usepackage{cancel}
\usepackage{url}

\definecolor{myc1}{HTML}{003049}
\definecolor{myc2}{HTML}{d62828}
\definecolor{myc3}{HTML}{f77f00}
\definecolor{myc4}{HTML}{6ca13b}

\definecolor{Q2}{HTML}{1f77b4}
\definecolor{Q1}{HTML}{ff7f0e}
\definecolor{Q3}{HTML}{2ca02c}

\definecolor{Q2}{HTML}{6ca13b}
\definecolor{Q1}{HTML}{6ca13b}
\definecolor{Q3}{HTML}{6ca13b}

\usepackage{tikz}
\usepackage{tikz-3dplot}
\usetikzlibrary{decorations.markings,arrows.meta,calc,shapes,intersections,backgrounds,patterns.meta,bending,angles,decorations.pathreplacing,decorations.pathmorphing}
\usepackage{xifthen}
\usepackage[normalem]{ulem}
\usepackage{pdflscape}
\usepackage{changepage}

\usepackage{pgfplots}
\usepgfplotslibrary{fillbetween}
\pgfplotsset{compat=1.12} % TikZ coordinates <-> axes coordinates


% Adjust the default font size and line spacing for the document
\AtBeginDocument{
  \fontsize{6pt}{10pt}\selectfont
  \setstretch{0.975}
}

% Customize section titles to be bold and use lmss
\titleformat*{\section}{\bfseries\fontfamily{lmss}\large\selectfont}
\titleformat*{\subsection}{\bfseries\fontfamily{lmss}\selectfont}
\titleformat*{\subsubsection}{\bfseries\fontfamily{lmss}\selectfont}

% Add 'S' prefix to figures, tables, and equations
\counterwithin{figure}{section}
\renewcommand{\thefigure}{S\arabic{figure}}
\counterwithin{table}{section}
\renewcommand{\thetable}{S\arabic{table}}
\counterwithin{equation}{section}
\renewcommand{\theequation}{S\arabic{equation}}

% Title, authors, and affiliations formatting
\usepackage{etoolbox} % Required for command redefinitions
\let\oldtitle\title
\renewcommand{\title}[1]{\oldtitle{{\fontfamily{lmss}\selectfont #1}}}
\let\oldauthor\author
\renewcommand{\author}[1]{\oldauthor{\large\fontfamily{lmss}\selectfont #1}}
\let\oldaffil\affil
\renewcommand{\affil}[1]{\oldaffil{\large\fontfamily{lmss}\selectfont #1}}

\newcommand{\cmark}{\ding{51}}% Checkmark
\newcommand{\xmark}{\ding{55}}% X mark

%----------------------------------------------------------------------
%----Helper code for dealing with external references----
% (by cyberSingularity at http://tex.stackexchange.com/a/69832/226)

\usepackage{xr}
% \usepackage[export]{adjustbox}
\makeatletter

\newcommand*{\addFileDependency}[1]{% argument=file name and extension
\typeout{(#1)}% latexmk will find this if $recorder=0
% however, in that case, it will ignore #1 if it is a .aux or 
% .pdf file etc and it exists! If it doesn't exist, it will appear 
% in the list of dependents regardless)
%
% Write the following if you want it to appear in \listfiles 
% --- although not really necessary and latexmk doesn't use this
%
\@addtofilelist{#1}
%
% latexmk will find this message if #1 doesn't exist (yet)
\IfFileExists{#1}{}{\typeout{No file #1.}}
}\makeatother

\newcommand*{\myexternaldocument}[1]{%
\externaldocument{#1}%
\addFileDependency{#1.tex}%
\addFileDependency{#1.aux}%
}
%------------End of helper code--------------

==> xx.tex <==


